Model-Adaptive Tool Necessity Reveals the Knowing-Doing Gap in LLM Tool Use

Large language models (LLMs) increasingly act as autonomous agents that must decide when to answer directly vs. when to invoke external tools. Prior work studying adaptive tool use has largely treated tool necessity as a model-agnostic property, annotated by human or LLM judge, and mostly cover cases where the answer is obvious (e.g., fetching the weather vs. paraphrasing text). However, tool necessity in the wild is more nuanced due to the divergence of capability boundaries across models: a problem solvable by a strong model on its own may still require tools for a weaker one. In this work, we introduce a model-adaptive definition of tool-necessity, grounded in each model's empirical performance. Following this definition, we compare the necessity against observed tool-call behavior across four models on arithmetic and factual QA dataset, and find substantial mismatches of 26.5-54.0% and 30.8-41.8%, respectively. To diagnose the failure, we decompose tool use into two stages: an internal cognition stage that reflects whether a model believes a tool is necessary, and an execution stage that determines whether the model actually makes a tool-call action. By probing the LLM hidden states, we find that both signals are often linearly decodable, yet their probe directions become nearly orthogonal in the late-layer, last-token regime that drives the next-token action. By tracing the trajectory of samples in the two-stage process, we further discover that the majority of mismatch is concentrated in the cognition-to-action transition, not in cognition itself. These results reveal a knowing-doing gap in LLM tool-use: improving tool-use reliability requires not only better recognition of when tools are needed, but also better translation of that recognition into action.

==> app/math_ds.tex <==
\section{Arithmetic dataset curation}
\label{app:arithmetic}
We generate math arithmetic problems grouped into three types. The easy group contains one-step addition/subtraction, short two-step chains, and small modulo problems. These give cases where a calculator is usually not needed. The larger short group keeps the expressions simple, but uses larger operands, including multi-digit subtraction, four-digit addition/subtraction, and two- or three-digit multiplication. These problems are still short enough to invite a direct answer, but they are more likely to cause digit errors. The multi-step group contains precedence chains, parenthesized expressions, multiplication chains, and long addition/subtraction chains. These examples test whether the model can track intermediate values and apply the order of operations, especially in cases that look simple but are easy to miscompute. Table~\ref{table:math-arithmetic} gives the problem families and their sampling shares.

\input{tabs-and-figs-tex/math_arithmetic}



==> app/system2.tex <==
\section{}

\input{tabs-and-figs-tex/2_stage_mcc_mismatch_change}

==> checklist.tex <==
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1--2 sentence) justification right after your answer (even for \answerNA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will also be asked to include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While \answerYes{} is generally preferable to \answerNo{}, it is perfectly acceptable to answer \answerNo{} provided a proper justification is given (e.g., error bars are not reported because it would be too computationally expensive'' or ``we were unable to find the license for the dataset we used''). In general, answering \answerNo{} or \answerNA{} is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}
    \item[] Justification: The abstract and introduction clearly state the findings regarding model-dependent tool necessity, the knowing-doing gap, and the two-stage cognition-execution modeling. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A \answerNo{} or \answerNA{} answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}
    \item[] Justification: The Limitations section is included in Appendix D.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper has no limitation while the answer \answerNo{} means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate ``Limitations'' section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper relies on empirical observations and definitions rather than formal theoretical proofs or theorems.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{}
    \item[] Justification: The paper provides details on the datasets used, models evaluated, inference parameters, and the specific formulations for linear probing.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item If the paper includes experiments, a \answerNo{} answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and\slash or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{}
    \item[] Justification: The code and data used is uploaded as supplementary material. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so \answerNo{} is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerYes{}
    \item[] Justification: All inference hyperparameters are given, and the exact train/test split ratios and the optimizer details for the linear probes are also specified.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{}
    \item[] Justification: The seeds are fixed in probe training for reproducibility, hence there is no statistical randomness in our probing results and analysis.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The authors should answer \answerYes{} if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g., negative error rates).
        \item If error bars are reported in tables or plots, the authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: The computation resource used is reported in Appendix C.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{}
    \item[] Justification: The research uses standard LLMs and benign datasets to analyze model behavior, presenting no foreseeable ethical violations.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer \answerNo, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNo{}
    \item[] Justification: This paper studies the reliable adaptive tool-calling in LLM agents, which to the best of our knowledge has no negative social impact. Positive impacts include better understanding of LLM tool-calling behaviors, which are trivial enough such that we believe no explicit elaboration is needed.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that there is no societal impact of the work performed.
        \item If the authors answer \answerNA{} or \answerNo, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate Deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper does not release high-risk models or sensitive scraped datasets; it analyzes existing open-weights models on standard benchmarks.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerNo{}
    \item[] Justification: We cite all the datasets and models but do not highlight their licenses in our paper, as they are widely used research dataset and models.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{}
    \item[] Justification: The newly curated Arithmetic dataset is well-documented in Appendix A, including problem families, proportions, and examples.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset\slash code\slash model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{}
    \item[] Justification: The research does not involve crowdsourcing or human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{}
    \item[] Justification: The research does not involve human subjects, so IRB approval is not applicable.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerNA{}
    \item[] Justification: LLMs are the subject of the empirical evaluation, not a non-standard tool used to generate the core research methodology.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy in the NeurIPS handbook for what should or should not be described.
    \end{itemize}

\end{enumerate}

==> secs/introduction.tex <==
\section{Introduction}

Large language models (LLMs) are increasingly deployed as autonomous or semi-autonomous agents that interact with external tools such as search engines, calculators, and APIs~\citep{parisi2022talm, schick2023toolformer, song2023restgpt, mialon2023augmented}. A central challenge in building reliable LLM agents is determining \textit{when} a model should rely on such tools versus answering directly~\citep{huang2024metatoolbenchmarklargelanguage, qian2025smartselfawareagenttool,wang2026positionagentinvokeexternal}. This decision is often framed as a form of meta-cognition~\citep{meta-cog-theory}: the model must assess its own knowledge and capabilities, recognize its limitations, and decide whether external assistance is required. Recent work~\citep{li2025adaptive,wang2026asatrainingfreerepresentationengineering} has suggested that LLMs possess surprisingly strong meta-cognitive abilities, with evidence drawn from probing internal representations in distinguishing tool-necessary and tool-unnecessary instances.

However, existing approaches~\citep{huang2024metatoolbenchmarklargelanguage,li2025adaptive,wang2026asatrainingfreerepresentationengineering} to studying tool use rely on a simplifying assumption: that tool necessity is an intrinsic, static property of a query. Under this paradigm, datasets are constructed by labeling queries as either “tool-necessary” (e.g., retrieving up-to-date information such as weather) or “tool-unnecessary” (e.g., paraphrasing text), typically based on human judgment or annotations from a stronger model. While convenient, this formulation conflates two distinct factors: the inherent difficulty of a query and the capabilities of the model tasked with solving it. In practice, \textbf{whether a tool is necessary depends not only on the query itself but also on the specific model’s knowledge and ability.} A query that is trivial for one model may be infeasible for another without external assistance.

This mismatch raises a fundamental question: \textit{are these measurements of LLM meta-cognition accurately measuring what they intend to measure?} If tool necessity is mis-specified, then observed performance may reflect artifacts of dataset construction rather than genuine meta-cognitive ability. In particular, models may appear competent simply because benchmarks emphasize extreme cases—queries that are either obviously solvable or obviously require tools—while neglecting the nuanced, model-dependent boundary between these regimes.

In this paper, we revisit the problem of tool-use decision making through a model-centric lens. We argue that tool necessity should be defined relative to a specific model, and we propose an empirical pipeline for doing so. Rather than relying on external annotations, we ground necessity in the observed capabilities of the model itself, distinguishing cases where the model unreliably answer queries without tool access and cases where the model consistently give correct answers on its own. This yields a more realistic and fine-grained partition of queries that better reflects the operational setting. 
Using this model-specific notion of tool necessity, we re-evaluate the meta-cognitive abilities of several LLMs. Our results challenge the optimistic conclusions of prior work: while some models still exhibit non-trivial meta-cognitive signals, overall performance is significantly weaker when evaluated under this more rigorous and context-sensitive definition. 
% This suggests that existing literature~\citep{li2025adaptive,wang2026asatrainingfreerepresentationengineering} may have overestimated the extent to which LLMs ``know what they don’t know''.

Taking a step further, we conduct a deeper analysis of failure modes in tool use. Even in models that demonstrate relatively strong meta-cognitive awareness, end-to-end tool-underuse and tool-overuse errors remain common. This raises a fundamental question: \textit{If a model have strong meta-cognitive awareness, what is causing its tool-underuse and tool-overuse errors?} To better understand these failures, we decouple two components of the decision-making process: (1) correctly recognizing that a tool is needed (meta-cognitive judgment), and (2) successfully acting on that recognition (execution). This distinction is analogous to the ``knowing–doing gap'' observed in the domain of LLM refusing harmful requests~\citep{zhao2025llmsencodeharmfulnessrefusal}, where models internally make correct assessments but fail to reflect that into the correct behavior.
Our mechanistic analysis reveals that these two components are \textbf{orthogonally separable} within model representations. Crucially, we find that execution failures—cases where the model appears to recognize the need for a tool but does not invoke it—account for a larger fraction of errors than incorrect necessity judgments. This shifts the focus from improving meta-cognitive awareness alone to addressing the reliability of executing tool-call actions.

Overall, our contributions are N-fold:

==> secs/introduction_v2.tex <==
\section{Introduction}
% \kr{we can use numbers for citations if needed}
\label{sec:intro}
Large language models (LLMs) are increasingly deployed as autonomous or semi-autonomous agents that interact with external tools such as search engines, calculators, and APIs~\citep{parisi2022talm, schick2023toolformer, song2023restgpt, mialon2023augmented}. A central challenge in building reliable LLM agents is determining \textit{when} a model should rely on such tools versus answering directly~\citep{huang2024metatoolbenchmarklargelanguage, qian2025smartselfawareagenttool,wang2026positionagentinvokeexternal}. This decision is often framed as a form of meta-cognition~\citep{meta-cog-theory}: the model must assess its own knowledge and capabilities, recognize its limitations, and decide whether external assistance is required. Recent work~\citep{li2025adaptive,wang2026asatrainingfreerepresentationengineering} has suggested that LLMs possess surprisingly strong meta-cognitive abilities, based on evidence that internal representations can distinguish between tool-necessary and tool-unnecessary queries.

However, two key assumptions underlie this optimistic view. First, prior work typically treats tool necessity as an intrinsic, static property of a query, labeling instances as either “tool-necessary” (e.g., retrieving up-to-date information) or “tool-unnecessary” (e.g., paraphrasing some given text). In practice, this notion is inherently model-dependent: whether a tool is required depends not only on the query, but also on the specific model’s knowledge and capabilities~\cite{wang2026positionagentinvokeexternal}. A question that is trivial for one model may be infeasible for another without external assistance. As a result, existing findings risk conflating task difficulty with model competence, potentially overstating meta-cognitive performance by focusing on clear-cut cases.

Second, even if tool necessity were perfectly specified, successful tool use requires more than accurate meta-cognitive judgment. A model must not only recognize when it needs a tool, but also reliably act on that recognition. Errors can therefore arise from two distinct sources: failures in \textit{judgment} (misidentifying whether a tool is needed) and failures in \textit{execution} (failing to invoke a tool despite recognizing the need). This distinction parallels the “knowing–doing gap” observed in other domains of LLM behavior~\citep{zhao2025llmsencodeharmfulnessrefusal}, where models internally encode correct assessments but fail to translate them into aligned actions.
\input{tabs-and-figs-tex/teaser_figure}

In this paper, we revisit tool-use decision making through these two complementary lenses. First, we introduce a \textbf{model-adaptive definition of tool necessity}, and propose a pipeline that ground tool necessity in the observed capabilities of a specific model rather than external annotations. By empirically identifying queries that a model can reliably answer without tools versus those it cannot, we obtain a more realistic and fine-grained partition of the problem space. Re-evaluating prior results under this definition reveals substantially weaker evidence of meta-cognitive ability than previously reported.

Second, we investigate the relationship between recognizing and acting on tool necessity. Through mechanistic analysis, we show that meta-cognitive judgment and tool-call execution are \textbf{orthogonally separable} within model representations. Importantly, we find that execution failures—cases where the model appears to correctly recognize the necessity for a tool but does not invoke it—account for a larger fraction of end-to-end errors than incorrect necessity judgments.

Together, these findings suggest that improving tool use in LLM agents requires addressing two distinct challenges: accurately characterizing when tools are needed, and ensuring that models can reliably act on that knowledge. Our results shift the focus from meta-cognitive awareness alone to the often-overlooked problem of execution, highlighting a key bottleneck in building dependable tool-augmented LLM systems.

Overall, our contributions are N-fold:



==> tabs-and-figs-tex/call_or_not_ampmeta.tex <==
\begin{table}[ht]
    \centering
    \caption{Breakdown of tool-call behavior across the four categories defined by the model-dependent necessity $n_f(x)$ and the observed action $a_f(z_f(x))$ \textbf{with the prompt amplifying meta-cognition}. Aligned cells (\textcolor{green!50!black}{N-C}: necessary-called, \textcolor{green!50!black}{UN-NC}: unnecessary-not-called) are shaded green; misaligned cells (\textcolor{red!70!black}{N-NC}, \textcolor{red!70!black}{UN-C}) are shaded red and together form the end-to-end mismatch $D(n_f(x), a_f(z_f(x)))$, summarized in the gray \textbf{Mis.}\ column. Each cell reports counts and the percentage of the per-model dataset total.}
    \label{tab:call_categories}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{l>{\columncolor{green!15}}c>{\columncolor{red!15}}c>{\columncolor{red!15}}c>{\columncolor{green!15}}c>{\columncolor{black!12}}c>{\columncolor{green!15}}c>{\columncolor{red!15}}c>{\columncolor{red!15}}c>{\columncolor{green!15}}c>{\columncolor{black!12}}c}
    \toprule
    \multirow{2}{*}{Model} & \multicolumn{5}{c}{Arithmetic} & \multicolumn{5}{c}{TruthfulQA} \\
    \cmidrule(lr){2-6} \cmidrule(lr){7-11}
     & N-C & N-NC & UN-C & UN-NC & \textbf{Mis.} & N-C & N-NC & UN-C & UN-NC & \textbf{Mis.} \\
    \midrule
    Qwen3-8B & 365 (9.1\%) & 213 (5.3\%) & 925 (23.1\%) & 2497 (62.4\%) & \textbf{28.4\%} & 64 (7.8\%) & 151 (18.5\%) & 94 (11.5\%) & 508 (62.2\%) & \textbf{30.0\%} \\
    Qwen3-4B & 143 (3.6\%) & 691 (17.3\%) & 309 (7.7\%) & 2857 (71.4\%) & \textbf{25.0\%} & 94 (11.5\%) & 162 (19.8\%) & 170 (20.8\%) & 391 (47.9\%) & \textbf{40.6\%} \\
    Llama-3.1-8B-Instruct & 519 (13.0\%) & 1104 (27.6\%) & 376 (9.4\%) & 2001 (50.0\%) & \textbf{37.0\%} & 121 (14.8\%) & 107 (13.1\%) & 188 (23.0\%) & 401 (49.1\%) & \textbf{36.1\%} \\
    Llama-3.2-3B-Instruct & 5 (0.1\%) & 2080 (52.0\%) & 1 (0.0\%) & 1914 (47.9\%) & \textbf{52.0\%} & 62 (7.6\%) & 160 (19.6\%) & 120 (14.7\%) & 475 (58.1\%) & \textbf{34.3\%} \\
    \bottomrule
    \end{tabular}%
    }
\end{table}

==> tabs-and-figs-tex/call_or_not_ampmetacog_and_exe.tex <==
\begin{table}[ht]
    \centering
    \caption{Breakdown of tool-call behavior across the four categories defined by the model-dependent necessity $n_f(x)$ and the observed action $a_f(z_f(x))$ \textbf{with the prompt amplifying meta-cognition and execution}. Aligned cells (\textcolor{green!50!black}{N-C}: necessary-called, \textcolor{green!50!black}{UN-NC}: unnecessary-not-called) are shaded green; misaligned cells (\textcolor{red!70!black}{N-NC}, \textcolor{red!70!black}{UN-C}) are shaded red and together form the end-to-end mismatch $D(n_f(x), a_f(z_f(x)))$, summarized in the gray \textbf{Mis.}\ column. Each cell reports counts and the percentage of the per-model dataset total.}
    \label{tab:call_categories}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{l>{\columncolor{green!15}}c>{\columncolor{red!15}}c>{\columncolor{red!15}}c>{\columncolor{green!15}}c>{\columncolor{black!12}}c>{\columncolor{green!15}}c>{\columncolor{red!15}}c>{\columncolor{red!15}}c>{\columncolor{green!15}}c>{\columncolor{black!12}}c}
    \toprule
    \multirow{2}{*}{Model} & \multicolumn{5}{c}{Arithmetic} & \multicolumn{5}{c}{TruthfulQA} \\
    \cmidrule(lr){2-6} \cmidrule(lr){7-11}
     & N-C & N-NC & UN-C & UN-NC & \textbf{Mis.} & N-C & N-NC & UN-C & UN-NC & \textbf{Mis.} \\
    \midrule
    Qwen3-8B & 350 (8.8\%) & 228 (5.7\%) & 888 (22.2\%) & 2534 (63.4\%) & \textbf{27.9\%} & 36 (4.4\%) & 179 (21.9\%) & 57 (7.0\%) & 545 (66.7\%) & \textbf{28.9\%} \\
    Qwen3-4B & 166 (4.2\%) & 668 (16.7\%) & 280 (7.0\%) & 2886 (72.2\%) & \textbf{23.7\%} & 125 (15.3\%) & 131 (16.0\%) & 247 (30.2\%) & 314 (38.4\%) & \textbf{46.3\%} \\
    Qwen2.5-7B-Instruct & 21 (0.5\%) & 1654 (41.4\%) & 15 (0.4\%) & 2310 (57.8\%) & \textbf{41.7\%} & 100 (12.2\%) & 101 (12.4\%) & 191 (23.4\%) & 425 (52.0\%) & \textbf{35.7\%} \\
    Llama-3.1-8B-Instruct & 542 (13.6\%) & 1081 (27.0\%) & 375 (9.4\%) & 2002 (50.0\%) & \textbf{36.4\%} & 132 (16.2\%) & 96 (11.8\%) & 192 (23.5\%) & 397 (48.6\%) & \textbf{35.3\%} \\
    Llama-3.2-3B-Instruct & 2 (0.1\%) & 2083 (52.1\%) & 7 (0.2\%) & 1908 (47.7\%) & \textbf{52.2\%} & 92 (11.3\%) & 130 (15.9\%) & 189 (23.1\%) & 406 (49.7\%) & \textbf{39.0\%} \\
    \bottomrule
    \end{tabular}%
    }
\end{table}
